Topological Data Analysis with $\epsilon$-net Induced Lazy Witness Complex

Topological data analysis computes and analyses topological features of the point clouds by constructing and studying a simplicial representation of the underlying topological structure. The enthusiasm that followed the initial successes of topological data analysis was curbed by the computational cost of constructing such simplicial representations. The lazy witness complex is a computationally feasible approximation of the underlying topological structure of a point cloud. It is built in reference to a subset of points, called landmarks, rather than considering all the points as in the \v{C}ech and Vietoris-Rips complexes. The choice and the number of landmarks dictate the effectiveness and efficiency of the approximation. We adopt the notion of $\epsilon$-cover to define $\epsilon$-net. We prove that $\epsilon$-net, as a choice of landmarks, is an $\epsilon$-approximate representation of the point cloud and the induced lazy witness complex is a $3$-approximation of the induced Vietoris-Rips complex. Furthermore, we propose three algorithms to construct $\epsilon$-net landmarks. We establish the relationship of these algorithms with the existing landmark selection algorithms. We empirically validate our theoretical claims. We empirically and comparatively evaluate the effectiveness, efficiency, and stability of the proposed algorithms on synthetic and real datasets.

==> tda_shortest.tex <==
\section{Topological Data Analysis}\label{sec:tda}%\vspace*{-1em}
Topological data analysis is the study of computational models for efficient and effective computation of topological features, such as homology classes, from different datasets, and representation of the topological features using different topological descriptors, such as persistence barcodes, for further analysis and application~\cite{edelsbrunner2010computational,otter2017roadmap}.
We represent the computational blocks of topological data analysis in Figure~\ref{fig:pipeline}.

\textbf{Computational models for Simplicial Representations.}\label{sec:model}
Topological data analysis constructs abstract simplicial complex representation from input data. An abstract simplicial complex consists of simplices. A $k$-simplex is a set of $(k+1)$ data points $\{v_0,v_1,\dots,v_k\}$. An \textbf{abstract simplicial complex}~\cite{edelsbrunner2010computational} $\mathcal{K}$ is a finite set of simplices such that all the subsets of a $k$-simplex belonging to $\mathcal{K}$ are also in $\mathcal{K}$, for any $k \in \mathbb{N} \cup \lbrace 0 \rbrace$. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figs/TDA_pipeline.pdf}
    \caption{\label{fig:pipeline}Components of topological data analysis.}%\vspace*{-1.7em}
\end{figure} 
In order to compute the abstract simplicial complex representation of the underlying space, researchers proposed several methods~\cite{otter2017roadmap}.
C\v ech complex produces the absolute simplicial complex representation.
Vietoris-Rips complex~\cite{edelsbrunner2010computational} produces the largest possible approximation of the C\v ech complex which is extensively used in topological data analysis literature~\cite{otter2017roadmap}.
 \begin{definition}[Vietoris-Rips complex~\cite{hausmann1995vietoris}]
The \textbf{Vietoris-Rips complex} $R_\epsilon(D)$, for a given dataset $D$ and real number $\epsilon > 0$, is an abstract simplicial complex representation consisting of such $k$-simplices, where any two points $v_i, v_j$ in any of these $k$-simplices have Euclidean distance $d(v_i,v_j) \leq \epsilon$. 
\end{definition}
A \v{C}ech complex $C_{\sqrt{2}\epsilon}$ always interleaves between two Vietoris-Rips complexes $R_\epsilon$ and $R_{2\epsilon}$~\cite{otter2017roadmap}. Hence, the simplices of the \v{C}ech complex are preserved in the Vietoris-Rips complex. Thus, we use the Vietoris-Rips complex as the baseline representation in this paper.

In the worst case, the number of simplices in the complex $R_\epsilon(D)$ grows exponentially with the number of data points $|D|$~\cite{otter2017roadmap,zomorodian2010fast}. Lazy witness complex~\cite{de2004topological} approximates the Vietoris-Rips complex by constructing the simplicial complexes over a subset of data points $L$, called \emph{landmarks}. 
Though this approximation leads to loss of topological features (\Cref{sec:experiment}), lazy witness complex captures a portion of the topological features of the underlying space depending on the choice of landmarks. 

The \textbf{lazy witness complex} $LW_\epsilon(D,L,\nu)$ of a dataset $D$ is a simplicial complex representation over a landmark set $L$ and a positive integer $\nu$, where $[v_iv_j], i \neq j$ is a $1$-simplex if and only if there exists a point $w \in D$ such that $\max(d(v_i,w),d(v_j,w)) \leq d^\nu_N(w) + \epsilon$,\footnote{$d^\nu_N(w)$ is the  geodesic distance from point $w \in V$ to its $\nu$-th nearest point in $L$.} and, $\sigma=[v_0 v_1\cdots v_k]$ is a $k$-simplex if and only if all pair of points $[v_iv_j] \subset \sigma$ are in $LW_\epsilon$.
% \end{definition}\vspace{-.5em}

The lazy witness complex $LW_\epsilon(D,L,0)$ for $L \subset V$ is the Vietoris-rips complex of the subgraph induced by $L$~\cite{silva2006selecting}. However, the lazy witness complexes grow exponentially with the number of landmarks $|L|$. Less number of landmarks accelerates computation while incurs more loss of topological features, which we illustrate in~\Cref{sec:experiment}. Thus, the choice of landmarks is dictated by the tradeoff between the approximation of topological features and computational resources available. We explore this in Sections~\ref{sec:graphtda} and~\ref{sec:experiment} as we propose landmark selection heuristics and experimentally evaluate their performance.

\textbf{Aggregation of Representations.} 
For small filtration parameter $\epsilon$, the Vietoris-Rips and lazy witness representations include small simplicial complexes with local connections.
For large $\epsilon$, they include large simplicial complexes with more global connections. 
Topological data analysis techniques construct a sequence of simplicial complex representations for a sequence of $\epsilon$'s so that it can include local and global connections. Such a sequence of simplicial complex representations is called a \emph{filtration}~\cite{carlssontda}. 
% A filtration~\cite{carlssontda} on dataset $D$ is a nested parameterized family of simplicial complexes $\mathcal{K}_{\epsilon_0} \subseteq \dots \subseteq \mathcal{K}_{\epsilon_i} \dots \subseteq \mathcal{K}_{\epsilon_{m}}$ where $\mathcal{K}_{\epsilon_i}$ is the simplicial complex representation of dataset $D$ with filtration parameter $\epsilon_i$ and 
% $0 \leq \epsilon_0<\cdots<\epsilon_{m} < \infty$. 

\textbf{Computation of Topological Features.}
Topological data analysis uses $k$-simplices to construct $k$-homology class~\cite{edelsbrunner2010computational,otter2017roadmap}. The $k$-homology classes are the intrinsic topological features of the data. We denote the set of k-homology classes as $H_k$. $H_k$ captures structural cavities created by the k-dimensional simplices of a simplicial complex~\cite{edelsbrunner2010computational,carlssontda}. 
As we increase the value of filtration parameter $\epsilon$, new simplices arrive, and the topological features (homology classes) start to appear in a simplicial complex. Some of the simplices get merged to the existing classes in a subsequent simplicial complex, and the rest persist indefinitely~\cite{edelsbrunner2010computational}. The life-time of a homology class is denoted by its appearance and merging filtration value pair $\epsilon_{b}$ and $\epsilon_{d}$ respectively. Such a pair constitutes a persistence interval $[\epsilon_{b},\epsilon_{d})$. The \emph{life-time} of such a homology class is defined as $\epsilon_{d}-\epsilon_{b}$. The persistence interval of an indefinitely persisting homology class is denoted as $[\epsilon_{b},\infty)$. Whether homology classes with longer life-time are more significant~\cite{carlssontda} than those with shorter life-time~\cite{Xia2014PersistentFolding} depends on the application. 

\textbf{Topological Descriptors} \label{subsec:tdadescriptors}
Topological descriptors~\cite{Carlsson:2004:PBS:1057432.1057449} represent persistence intervals to draw qualitative and quantitative inference about the topological features. They differ from each other by the way they represent the intervals, as well as the kind of analysis one, can do on them.

\emph{Persistence diagram~\cite{edelsbrunner2010computational}} is a descriptor that represents a collection of persistence intervals at dimension $k$ as a multiset of points in the extended plane $\mathbb{R}_+^2$. 
\emph{Persistence barcode~\cite{collins2004barcode}} descriptor represents each interval as a horizontal bar in the extended plane $\mathbb{R}_+^2$ where the horizontal axis represents different values of filtration parameter. The intervals at dimension $k$ are stacked up. There is no canonical ordering of the bars. We use persistence barcode as the topological descriptor in this paper (Section~\ref{sec:experiment}). We order the bars in ascending order of their life-time and birth filtration value for consistency.
